Compression of Deep Learning Models for Text: A Survey

In recent years, the fields of natural language processing (NLP) and information retrieval (IR) have made tremendous progress thanksto deep learning models like Recurrent Neural Networks (RNNs), Gated Recurrent Units (GRUs) and Long Short-Term Memory (LSTMs)networks, and Transformer [120] based models like Bidirectional Encoder Representations from Transformers (BERT) [24], GenerativePre-training Transformer (GPT-2) [94], Multi-task Deep Neural Network (MT-DNN) [73], Extra-Long Network (XLNet) [134], Text-to-text transfer transformer (T5) [95], T-NLG [98] and GShard [63]. But these models are humongous in size. On the other hand,real world applications demand small model size, low response times and low computational power wattage. In this survey, wediscuss six different types of methods (Pruning, Quantization, Knowledge Distillation, Parameter Sharing, Tensor Decomposition, andSub-quadratic Transformer based methods) for compression of such models to enable their deployment in real industry NLP projects.Given the critical need of building applications with efficient and small models, and the large amount of recently published work inthis area, we believe that this survey organizes the plethora of work done by the 'deep learning for NLP' community in the past fewyears and presents it as a coherent story.

==> bibliography.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{100}
\scriptsize
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{vaswani2017attention}
A.~Vaswani, N.~Shazeer, N.~Parmar, J.~Uszkoreit, L.~Jones, A.~N. Gomez,
  {\L}.~Kaiser, and I.~Polosukhin, ``Attention is all you need,'' in
  \emph{NIPS}, 2017, pp. 5998--6008.

\bibitem{devlin2018bert}
J.~Devlin, M.-W. Chang, K.~Lee, and K.~Toutanova, ``Bert: Pre-training of deep
  bidirectional transformers for language understanding,''
  \emph{arXiv:1810.04805}, 2018.

\bibitem{wang2019glue}
A.~Wang, A.~Singh, J.~Michael, F.~Hill, O.~Levy, and S.~R. Bowman, ``{GLUE}: A
  multi-task benchmark and analysis platform for natural language
  understanding,'' in \emph{ICLR}, 2019.

\bibitem{wang2019superglue}
A.~Wang, Y.~Pruksachatkun, N.~Nangia, A.~Singh, J.~Michael, F.~Hill, O.~Levy,
  and S.~R. Bowman, ``Super{GLUE}: A stickier benchmark for general-purpose
  language understanding systems,'' \emph{1905.00537}, 2019.

\bibitem{radford2019language}
A.~Radford, J.~Wu, R.~Child, D.~Luan, D.~Amodei, and I.~Sutskever, ``Language
  models are unsupervised multitask learners,'' \emph{OpenAI Blog}, vol.~1,
  no.~8, 2019.

\bibitem{liu2019multi}
X.~Liu, P.~He, W.~Chen, and J.~Gao, ``Multi-task deep neural networks for
  natural language understanding,'' \emph{arXiv:1901.11504}, 2019.

\bibitem{yang2019xlnet}
Z.~Yang, Z.~Dai, Y.~Yang, J.~Carbonell, R.~Salakhutdinov, and Q.~V. Le,
  ``Xlnet: Generalized autoregressive pretraining for language understanding,''
  \emph{arXiv:1906.08237}, 2019.

\bibitem{shoeybi2019megatron}
M.~Shoeybi, M.~Patwary, R.~Puri, P.~LeGresley, J.~Casper, and B.~Catanzaro,
  ``Megatron-lm: Training multi-billion parameter language models using gpu
  model parallelism,'' \emph{arXiv:1909.08053}, 2019.

\bibitem{raffel2019exploring}
C.~Raffel, N.~Shazeer, A.~Roberts, K.~Lee, S.~Narang, M.~Matena, Y.~Zhou,
  W.~Li, and P.~J. Liu, ``Exploring the limits of transfer learning with a
  unified text-to-text transformer,'' \emph{arXiv:1910.10683}, 2019.

\bibitem{rosset2019turing}
C.~Rosset, ``Turing-nlg: A 17-billion-parameter language model by microsoft,''
  \emph{Microsoft Blog}, 2019.

\bibitem{lepikhin2020gshard}
D.~Lepikhin, H.~Lee, Y.~Xu, D.~Chen, O.~Firat, Y.~Huang, M.~Krikun, N.~Shazeer,
  and Z.~Chen, ``Gshard: Scaling giant models with conditional computation and
  automatic sharding,'' \emph{arXiv:2006.16668}, 2020.

\bibitem{bianco2018benchmark}
S.~Bianco, R.~Cadene, L.~Celona, and P.~Napoletano, ``Benchmark analysis of
  representative deep neural network architectures,'' \emph{IEEE Access},
  vol.~6, pp. 64\,270--64\,277, 2018.

\bibitem{sanh2019distilbert}
V.~Sanh, L.~Debut, J.~Chaumond, and T.~Wolf, ``Distilbert, a distilled version
  of bert: smaller, faster, cheaper and lighter,'' \emph{arXiv:1910.01108},
  2019.

\bibitem{han2016eie}
S.~Han, X.~Liu, H.~Mao, J.~Pu, A.~Pedram, M.~A. Horowitz, and W.~J. Dally,
  ``Eie: efficient inference engine on compressed deep neural network,''
  \emph{ACM SIGARCH Computer Architecture News}, vol.~44, no.~3, pp. 243--254,
  2016.

\bibitem{diamos2016persistent}
G.~Diamos, S.~Sengupta, B.~Catanzaro, M.~Chrzanowski, A.~Coates, E.~Elsen,
  J.~Engel, A.~Hannun, and S.~Satheesh, ``Persistent rnns: Stashing recurrent
  weights on-chip,'' in \emph{ICML}, 2016, pp. 2024--2033.

\bibitem{denil2013predicting}
M.~Denil, B.~Shakibi, L.~Dinh, M.~Ranzato, and N.~De~Freitas, ``Predicting
  parameters in deep learning,'' in \emph{NIPS}, 2013, pp. 2148--2156.

\bibitem{cheng2017survey}
Y.~Cheng, D.~Wang, P.~Zhou, and T.~Zhang, ``A survey of model compression and
  acceleration for deep neural networks,'' \emph{arXiv:1710.09282}, 2017.

\bibitem{deng2020model}
L.~Deng, G.~Li, S.~Han, L.~Shi, and Y.~Xie, ``Model compression and hardware
  acceleration for neural networks: A comprehensive survey,'' \emph{IEEE}, vol.
  108, no.~4, pp. 485--532, 2020.

\bibitem{walsh2013peter}
C.~A. Walsh, ``Peter huttenlocher (1931--2013),'' \emph{Nature}, vol. 502, no.
  7470, pp. 172--172, 2013.

\bibitem{zhu2017prune}
M.~Zhu and S.~Gupta, ``To prune, or not to prune: exploring the efficacy of
  pruning for model compression,'' \emph{arXiv:1710.01878}, 2017.

\bibitem{lecun1990optimal}
Y.~LeCun, J.~S. Denker, and S.~A. Solla, ``Optimal brain damage,'' in
  \emph{NIPS}, 1990, pp. 598--605.

\bibitem{hassibi1993second}
B.~Hassibi and D.~G. Stork, ``Second order derivatives for network pruning:
  Optimal brain surgeon,'' in \emph{NIPS}, 1993, pp. 164--171.

\bibitem{han2015deep}
S.~Han, H.~Mao, and W.~J. Dally, ``Deep compression: Compressing deep neural
  networks with pruning, trained quantization and huffman coding,''
  \emph{arXiv:1510.00149}, 2015.

\bibitem{see2016compression}
A.~See, M.-T. Luong, and C.~D. Manning, ``Compression of neural machine
  translation models via pruning,'' \emph{arXiv:1606.09274}, 2016.

\bibitem{han2015learning}
S.~Han, J.~Pool, J.~Tran, and W.~Dally, ``Learning both weights and connections
  for efficient neural network,'' in \emph{NIPS}, 2015, pp. 1135--1143.

\bibitem{narang2017exploring}
S.~Narang, E.~Elsen, G.~Diamos, and S.~Sengupta, ``Exploring sparsity in
  recurrent neural networks,'' \emph{arXiv:1704.05119}, 2017.

\bibitem{cheong2019transformers}
R.~Cheong and R.~Daniel, ``transformers. zip: Compressing transformers with
  pruning and quantization,'' Technical report, Stanford University, Stanford,
  California, 2019., Tech. Rep., 2019.

\bibitem{guo2019reweighted}
F.-M. Guo, S.~Liu, F.~S. Mungall, X.~Lin, and Y.~Wang, ``Reweighted proximal
  pruning for large-scale language representation,'' \emph{arXiv:1909.12486},
  2019.

\bibitem{han2016dsd}
S.~Han, J.~Pool, S.~Narang, H.~Mao, E.~Gong, S.~Tang, E.~Elsen, P.~Vajda,
  M.~Paluri, J.~Tran \emph{et~al.}, ``Dsd: Dense-sparse-dense training for deep
  neural networks,'' \emph{arXiv:1607.04381}, 2016.

\bibitem{dai2018grow}
X.~Dai, H.~Yin, and N.~K. Jha, ``Grow and prune compact, fast, and accurate
  lstms,'' \emph{arXiv:1805.11797}, 2018.

\bibitem{he2014reshaping}
T.~He, Y.~Fan, Y.~Qian, T.~Tan, and K.~Yu, ``Reshaping deep neural network for
  fast decoding by node-pruning,'' in \emph{ICASSP}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2014, pp. 245--249.

\bibitem{murray2015auto}
K.~Murray and D.~Chiang, ``Auto-sizing neural networks: With applications to
  n-gram language models,'' \emph{arXiv:1508.05051}, 2015.

\bibitem{pan2016dropneuron}
W.~Pan, H.~Dong, and Y.~Guo, ``Dropneuron: Simplifying the structure of deep
  neural networks,'' \emph{arXiv:1606.07326}, 2016.

\bibitem{srinivas2015data}
S.~Srinivas and R.~V. Babu, ``Data-free parameter pruning for deep neural
  networks,'' \emph{arXiv:1507.06149}, 2015.

\bibitem{narang2017block}
S.~Narang, E.~Undersander, and G.~Diamos, ``Block-sparse recurrent neural
  networks,'' \emph{arXiv:1711.02782}, 2017.

\bibitem{cao2019efficient}
S.~Cao, C.~Zhang, Z.~Yao, W.~Xiao, L.~Nie, D.~Zhan, Y.~Liu, M.~Wu, and
  L.~Zhang, ``Efficient and effective sparse lstm on fpga with bank-balanced
  sparsity,'' in \emph{SIGDA Intl. Symp. on FPGA}.\hskip 1em plus 0.5em minus
  0.4em\relax ACM, 2019, pp. 63--72.

\bibitem{michel2019sixteen}
P.~Michel, O.~Levy, and G.~Neubig, ``Are sixteen heads really better than
  one?'' \emph{arXiv:1905.10650}, 2019.

\bibitem{voita2019analyzing}
E.~Voita, D.~Talbot, F.~Moiseev, R.~Sennrich, and I.~Titov, ``Analyzing
  multi-head self-attention: Specialized heads do the heavy lifting, the rest
  can be pruned,'' \emph{arXiv:1905.09418}, 2019.

\bibitem{ding2017visualizing}
Y.~Ding, Y.~Liu, H.~Luan, and M.~Sun, ``Visualizing and understanding neural
  machine translation,'' in \emph{ACL}, 2017, pp. 1150--1159.

\bibitem{fan2019reducing}
A.~Fan, E.~Grave, and A.~Joulin, ``Reducing transformer depth on demand with
  structured dropout,'' \emph{arXiv:1909.11556}, 2019.

\bibitem{prasanna2020bert}
S.~Prasanna, A.~Rogers, and A.~Rumshisky, ``When bert plays the lottery, all
  tickets are winning,'' \emph{arXiv:2005.00561}, 2020.

\bibitem{bartol2015hippocampal}
T.~M. Bartol, C.~Bromer, J.~Kinney, M.~A. Chirillo, J.~N. Bourne, K.~M. Harris,
  and T.~J. Sejnowski, ``Hippocampal spine head sizes are highly precise,''
  \emph{bioRxiv}, p. 016329, 2015.

\bibitem{linden2018think}
D.~J. Linden, \emph{Think Tank: Forty Neuroscientists Explore the Biological
  Roots of Human Experience}.\hskip 1em plus 0.5em minus 0.4em\relax Yale
  University Press, 2018.

\bibitem{hubara2017quantized}
I.~Hubara, M.~Courbariaux, D.~Soudry, R.~El-Yaniv, and Y.~Bengio, ``Quantized
  neural networks: Training neural networks with low precision weights and
  activations,'' \emph{JMLR}, vol.~18, no.~1, pp. 6869--6898, 2017.

\bibitem{lam2018word2bits}
M.~Lam, ``Word2bits-quantized word vectors,'' \emph{arXiv:1803.05651}, 2018.

\bibitem{courbariaux2015binaryconnect}
M.~Courbariaux, Y.~Bengio, and J.-P. David, ``Binaryconnect: Training deep
  neural networks with binary weights during propagations,'' in \emph{NIPS},
  2015, pp. 3123--3131.

\bibitem{bengio2013estimating}
Y.~Bengio, N.~L{\'e}onard, and A.~Courville, ``Estimating or propagating
  gradients through stochastic neurons for conditional computation,''
  \emph{arXiv:1308.3432}, 2013.

\bibitem{lin2015neural}
Z.~Lin, M.~Courbariaux, R.~Memisevic, and Y.~Bengio, ``Neural networks with few
  multiplications,'' \emph{arXiv:1510.03009}, 2015.

\bibitem{hubara2016binarized}
I.~Hubara, M.~Courbariaux, D.~Soudry, R.~El-Yaniv, and Y.~Bengio, ``Binarized
  neural networks,'' in \emph{NIPS}, 2016, pp. 4107--4115.

\bibitem{rastegari2016xnor}
M.~Rastegari, V.~Ordonez, J.~Redmon, and A.~Farhadi, ``Xnor-net: Imagenet
  classification using binary convolutional neural networks,'' in
  \emph{ECCV}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2016, pp.
  525--542.

\bibitem{hou2016loss}
L.~Hou, Q.~Yao, and J.~T. Kwok, ``Loss-aware binarization of deep networks,''
  \emph{arXiv:1611.01600}, 2016.

\bibitem{lee2014proximal}
J.~D. Lee, Y.~Sun, and M.~A. Saunders, ``Proximal newton-type methods for
  minimizing composite functions,'' \emph{J. Optimization}, vol.~24, no.~3, pp.
  1420--1443, 2014.

\bibitem{ott2016recurrent}
J.~Ott, Z.~Lin, Y.~Zhang, S.-C. Liu, and Y.~Bengio, ``Recurrent neural networks
  with limited numerical precision,'' \emph{arXiv:1608.06902}, 2016.

\bibitem{alom2018effective}
M.~Z. Alom, A.~T. Moody, N.~Maruyama, B.~C. Van~Essen, and T.~M. Taha,
  ``Effective quantization approaches for recurrent neural networks,'' in
  \emph{IJCNN}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 1--8.

\bibitem{li2016ternary}
F.~Li, B.~Zhang, and B.~Liu, ``Ternary weight networks,''
  \emph{arXiv:1605.04711}, 2016.

\bibitem{hwang2014fixed}
K.~Hwang and W.~Sung, ``Fixed-point feedforward deep neural network design
  using weights+ 1, 0, and- 1,'' in \emph{SiPS}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2014, pp. 1--6.

\bibitem{lloyd1982least}
S.~Lloyd, ``Least squares quantization in pcm,'' \emph{Tran. on information
  theory}, vol.~28, no.~2, pp. 129--137, 1982.

\bibitem{zhu2016trained}
C.~Zhu, S.~Han, H.~Mao, and W.~J. Dally, ``Trained ternary quantization,''
  \emph{arXiv:1612.01064}, 2016.

\bibitem{wang2018hitnet}
P.~Wang, X.~Xie, L.~Deng, G.~Li, D.~Wang, and Y.~Xie, ``Hitnet: hybrid ternary
  recurrent neural network,'' in \emph{NIPS}, 2018, pp. 604--614.

\bibitem{he2016effective}
Q.~He, H.~Wen, S.~Zhou, Y.~Wu, C.~Yao, X.~Zhou, and Y.~Zou, ``Effective
  quantization methods for recurrent neural networks,''
  \emph{arXiv:1611.10176}, 2016.

\bibitem{zhou2017balanced}
S.-C. Zhou, Y.-Z. Wang, H.~Wen, Q.-Y. He, and Y.-H. Zou, ``Balanced
  quantization: An effective and efficient approach to quantized neural
  networks,'' \emph{J. of Computer Science and Technology}, vol.~32, no.~4, pp.
  667--682, 2017.

\bibitem{muller2015rounding}
L.~K. Muller and G.~Indiveri, ``Rounding methods for neural networks with low
  resolution synaptic weights,'' \emph{arXiv:1504.05767}, 2015.

\bibitem{gong2014compressing}
Y.~Gong, L.~Liu, M.~Yang, and L.~Bourdev, ``Compressing deep convolutional
  networks using vector quantization,'' \emph{arXiv:1412.6115}, 2014.

\bibitem{guo2017network}
Y.~Guo, A.~Yao, H.~Zhao, and Y.~Chen, ``Network sketching: Exploiting binary
  structure in deep cnns,'' in \emph{CVPR}, 2017, pp. 5955--5963.

\bibitem{xu2018alternating}
C.~Xu, J.~Yao, Z.~Lin, W.~Ou, Y.~Cao, Z.~Wang, and H.~Zha, ``Alternating
  multi-bit quantization for recurrent neural networks,''
  \emph{arXiv:1802.00150}, 2018.

\bibitem{mikolov2013word2vec}
T.~Mikolov, K.~Chen, G.~Corrado, J.~Dean, L.~Sutskever, and G.~Zweig,
  ``word2vec,'' \emph{URL https://code. google. com/p/word2vec}, vol.~22, 2013.

\bibitem{shen2019q}
S.~Shen, Z.~Dong, J.~Ye, L.~Ma, Z.~Yao, A.~Gholami, M.~W. Mahoney, and
  K.~Keutzer, ``Q-bert: Hessian based ultra low precision quantization of
  bert,'' \emph{arXiv:1909.05840}, 2019.

\bibitem{ba2014deep}
J.~Ba and R.~Caruana, ``Do deep nets really need to be deep?'' in \emph{NIPS},
  2014, pp. 2654--2662.

\bibitem{sau2016deep}
B.~B. Sau and V.~N. Balasubramanian, ``Deep model compression: Distilling
  knowledge from noisy teachers,'' \emph{arXiv:1610.09650}, 2016.

\bibitem{hinton2015distilling}
G.~Hinton, O.~Vinyals, and J.~Dean, ``Distilling the knowledge in a neural
  network,'' \emph{arXiv:1503.02531}, 2015.

\bibitem{czarnecki2017sobolev}
W.~M. Czarnecki, S.~Osindero, M.~Jaderberg, G.~Swirszcz, and R.~Pascanu,
  ``Sobolev training for neural networks,'' in \emph{NIPS}, 2017, pp.
  4278--4287.

\bibitem{mishra2017apprentice}
A.~Mishra and D.~Marr, ``Apprentice: Using knowledge distillation techniques to
  improve low-precision network accuracy,'' \emph{arXiv:1711.05852}, 2017.

\bibitem{polino2018model}
A.~Polino, R.~Pascanu, and D.~Alistarh, ``Model compression via distillation
  and quantization,'' \emph{arXiv:1802.05668}, 2018.

\bibitem{romero2014fitnets}
A.~Romero, N.~Ballas, S.~E. Kahou, A.~Chassang, C.~Gatta, and Y.~Bengio,
  ``Fitnets: Hints for thin deep nets,'' \emph{arXiv:1412.6550}, 2014.

\bibitem{yim2017gift}
J.~Yim, D.~Joo, J.~Bae, and J.~Kim, ``A gift from knowledge distillation: Fast
  optimization, network minimization and transfer learning,'' in \emph{CVPR},
  2017, pp. 4133--4141.

\bibitem{mcclure2016representational}
P.~McClure and N.~Kriegeskorte, ``Representational distance learning for deep
  neural networks,'' \emph{Frontiers in computational neuroscience}, vol.~10,
  p. 131, 2016.

\bibitem{kim2016sequence}
Y.~Kim and A.~M. Rush, ``Sequence-level knowledge distillation,''
  \emph{arXiv:1606.07947}, 2016.

\bibitem{freitag2017ensemble}
M.~Freitag, Y.~Al-Onaizan, and B.~Sankaran, ``Ensemble distillation for neural
  machine translation,'' \emph{arXiv:1702.01802}, 2017.

\bibitem{zhang2018deep}
Y.~Zhang, T.~Xiang, T.~M. Hospedales, and H.~Lu, ``Deep mutual learning,'' in
  \emph{CVPR}, 2018, pp. 4320--4328.

\bibitem{anil2018large}
R.~Anil, G.~Pereyra, A.~Passos, R.~Ormandi, G.~E. Dahl, and G.~E. Hinton,
  ``Large scale distributed neural network training through online
  distillation,'' \emph{arXiv:1804.03235}, 2018.

\bibitem{mirzadeh2019improved}
S.-I. Mirzadeh, M.~Farajtabar, A.~Li, N.~Levine, A.~Matsukawa, and
  H.~Ghasemzadeh, ``Improved knowledge distillation via teacher assistant,''
  \emph{arXiv:1902.03393}, 2019.

\bibitem{you2017learning}
S.~You, C.~Xu, C.~Xu, and D.~Tao, ``Learning from multiple teacher networks,''
  in \emph{KDD}, 2017, pp. 1285--1294.

\bibitem{tan2019multilingual}
X.~Tan, Y.~Ren, D.~He, T.~Qin, Z.~Zhao, and T.-Y. Liu, ``Multilingual neural
  machine translation with knowledge distillation,'' \emph{arXiv:1902.10461},
  2019.

\bibitem{heo2019knowledge}
B.~Heo, M.~Lee, S.~Yun, and J.~Y. Choi, ``Knowledge distillation with
  adversarial samples supporting decision boundary,'' in \emph{AAAI}, vol.~33,
  2019, pp. 3771--3778.

\bibitem{xu2017training}
Z.~Xu, Y.-C. Hsu, and J.~Huang, ``Training shallow and thin networks for
  acceleration via knowledge distillation with conditional adversarial
  networks,'' \emph{arXiv:1709.00513}, 2017.

\bibitem{wang2018kdgan}
X.~Wang, R.~Zhang, Y.~Sun, and J.~Qi, ``Kdgan: Knowledge distillation with
  generative adversarial networks,'' in \emph{NIPS}, 2018, pp. 775--786.

\bibitem{zhao2019extreme}
S.~Zhao, R.~Gupta, Y.~Song, and D.~Zhou, ``Extreme language model compression
  with optimal subwords and shared projections,'' \emph{arXiv:1909.11687},
  2019.

\bibitem{sun2019patient}
S.~Sun, Y.~Cheng, Z.~Gan, and J.~Liu, ``Patient knowledge distillation for bert
  model compression,'' \emph{arXiv:1908.09355}, 2019.

\bibitem{jiao2019tinybert}
X.~Jiao, Y.~Yin, L.~Shang, X.~Jiang, X.~Chen, L.~Li, F.~Wang, and Q.~Liu,
  ``Tinybert: Distilling bert for natural language understanding,''
  \emph{arXiv:1909.10351}, 2019.

\bibitem{liu2019improving}
X.~Liu, P.~He, W.~Chen, and J.~Gao, ``Improving multi-task deep neural networks
  via knowledge distillation for natural language understanding,''
  \emph{arXiv:1904.09482}, 2019.

\bibitem{wang2020minilm}
W.~Wang, F.~Wei, L.~Dong, H.~Bao, N.~Yang, and M.~Zhou, ``Minilm: Deep
  self-attention distillation for task-agnostic compression of pre-trained
  transformers,'' \emph{arXiv:2002.10957}, 2020.

\bibitem{tang2019distilling}
R.~Tang, Y.~Lu, L.~Liu, L.~Mou, O.~Vechtomova, and J.~Lin, ``Distilling
  task-specific knowledge from bert into simple neural networks,''
  \emph{arXiv:1903.12136}, 2019.

\bibitem{mukherjee2020xtremedistil}
S.~Mukherjee and A.~H. Awadallah, ``Xtremedistil: Multi-stage distillation for
  massive multilingual models,'' in \emph{ACL}, 2020, pp. 2221--2234.

\bibitem{ling2015finding}
W.~Ling, T.~Lu{\'\i}s, L.~Marujo, R.~F. Astudillo, S.~Amir, C.~Dyer, A.~W.
  Black, and I.~Trancoso, ``Finding function in form: Compositional character
  models for open vocabulary word representation,'' \emph{arXiv:1508.02096},
  2015.

\bibitem{jozefowicz2016exploring}
R.~Jozefowicz, O.~Vinyals, M.~Schuster, N.~Shazeer, and Y.~Wu, ``Exploring the
  limits of language modeling,'' \emph{arXiv:1602.02410}, 2016.

\bibitem{kim2016character}
Y.~Kim, Y.~Jernite, D.~Sontag, and A.~M. Rush, ``Character-aware neural
  language models,'' in \emph{AAAI}, 2016.

\bibitem{chen2015compressing}
W.~Chen, J.~Wilson, S.~Tyree, K.~Weinberger, and Y.~Chen, ``Compressing neural
  networks with the hashing trick,'' in \emph{ICML}, 2015, pp. 2285--2294.

\bibitem{lu2016learning}
Z.~Lu, V.~Sindhwani, and T.~N. Sainath, ``Learning compact recurrent neural
  networks,'' in \emph{ICASSP}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2016, pp. 5960--5964.

\bibitem{tay2019lightweight}
Y.~Tay, A.~Zhang, L.~A. Tuan, J.~Rao, S.~Zhang, S.~Wang, J.~Fu, and S.~C. Hui,
  ``Lightweight and efficient neural natural language processing with
  quaternion networks,'' \emph{arXiv:1906.04393}, 2019.

\bibitem{chen2016compressing}
Y.~Chen, L.~Mou, Y.~Xu, G.~Li, and Z.~Jin, ``Compressing neural language models
  by sparse word representations,'' \emph{arXiv:1610.03950}, 2016.

\bibitem{li2016lightrnn}
X.~Li, T.~Qin, J.~Yang, and T.-Y. Liu, ``Lightrnn: Memory and
  computation-efficient recurrent neural networks,'' in \emph{NIPS}, 2016, pp.
  4385--4393.

\bibitem{suzuki2016learning}
J.~Suzuki and M.~Nagata, ``Learning compact neural word embeddings by parameter
  space sharing.'' in \emph{IJCAI}, 2016, pp. 2046--2052.

\bibitem{li2018slim}
Z.~Li, R.~Kulhanek, S.~Wang, Y.~Zhao, and S.~Wu, ``Slim embedding layers for
  recurrent neural language models,'' in \emph{AAAI}, 2018.

\bibitem{lan2019albert}
Z.~Lan, M.~Chen, S.~Goodman, K.~Gimpel, P.~Sharma, and R.~Soricut, ``Albert: A
  lite bert for self-supervised learning of language representations,''
  \emph{arXiv:1909.11942}, 2019.

\bibitem{dehghani2018universal}
M.~Dehghani, S.~Gouws, O.~Vinyals, J.~Uszkoreit, and {\L}.~Kaiser, ``Universal
  transformers,'' \emph{arXiv:1807.03819}, 2018.

\bibitem{bai2019deep}
S.~Bai, J.~Z. Kolter, and V.~Koltun, ``Deep equilibrium models,''
  \emph{arXiv:1909.01377}, 2019.

\bibitem{oseledets2011tensor}
I.~V. Oseledets, ``Tensor-train decomposition,'' \emph{SIAM J. on Scientific
  Computing}, vol.~33, no.~5, pp. 2295--2317, 2011.

\bibitem{carroll1970analysis}
J.~D. Carroll and J.-J. Chang, ``Analysis of individual differences in
  multidimensional scaling via an n-way generalization of “eckart-young”
  decomposition,'' \emph{Psychometrika}, vol.~35, no.~3, pp. 283--319, 1970.

\bibitem{tucker1966some}
L.~R. Tucker, ``Some mathematical notes on three-mode factor analysis,''
  \emph{Psychometrika}, vol.~31, no.~3, pp. 279--311, 1966.

\bibitem{prabhavalkar2016compression}
R.~Prabhavalkar, O.~Alsharif, A.~Bruguier, and L.~McGraw, ``On the compression
  of recurrent neural networks with an application to lvcsr acoustic modeling
  for embedded speech recognition,'' in \emph{ICASSP}.\hskip 1em plus 0.5em
  minus 0.4em\relax IEEE, 2016, pp. 5970--5974.

\bibitem{sak2014long}
H.~Sak, A.~Senior, and F.~Beaufays, ``Long short-term memory based recurrent
  neural network architectures for large vocabulary speech recognition,''
  \emph{arXiv:1402.1128}, 2014.

\bibitem{faruqui2015sparse}
M.~Faruqui, Y.~Tsvetkov, D.~Yogatama, C.~Dyer, and N.~Smith, ``Sparse
  overcomplete word vector representations,'' \emph{arXiv:1506.02004}, 2015.

\bibitem{shu2017compressing}
R.~Shu and H.~Nakayama, ``Compressing word embeddings via deep compositional
  code learning,'' \emph{arXiv:1711.01068}, 2017.

\bibitem{wang2019structured}
Z.~Wang, J.~Wohlwend, and T.~Lei, ``Structured pruning of large language
  models,'' \emph{arXiv:1910.04732}, 2019.

\bibitem{chen2015strategies}
W.~Chen, D.~Grangier, and M.~Auli, ``Strategies for training large vocabulary
  neural language models,'' \emph{arXiv:1512.04906}, 2015.

\bibitem{variani2019west}
E.~Variani, A.~T. Suresh, and M.~Weintraub, ``West: Word encoded sequence
  transducers,'' in \emph{ICASSP}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2019, pp. 7340--7344.

\bibitem{tjandra2017compressing}
A.~Tjandra, S.~Sakti, and S.~Nakamura, ``Compressing recurrent neural network
  with tensor train,'' in \emph{IJCNN}.\hskip 1em plus 0.5em minus 0.4em\relax
  IEEE, 2017, pp. 4451--4458.

\bibitem{khrulkov2019tensorized}
V.~Khrulkov, O.~Hrinchuk, L.~Mirvakhabova, and I.~Oseledets, ``Tensorized
  embedding layers for efficient model compression,'' \emph{arXiv:1901.10787},
  2019.

\bibitem{ye2018learning}
J.~Ye, L.~Wang, G.~Li, D.~Chen, S.~Zhe, X.~Chu, and Z.~Xu, ``Learning compact
  recurrent neural networks with block-term tensor decomposition,'' in
  \emph{CVPR}, 2018, pp. 9378--9387.

\bibitem{ma2019tensorized}
X.~Ma, P.~Zhang, S.~Zhang, N.~Duan, Y.~Hou, D.~Song, and M.~Zhou, ``A
  tensorized transformer for language modeling,'' \emph{arXiv:1906.09777},
  2019.

\bibitem{child2019generating}
R.~Child, S.~Gray, A.~Radford, and I.~Sutskever, ``Generating long sequences
  with sparse transformers,'' \emph{arXiv:1904.10509}, 2019.

\bibitem{guo2019star}
Q.~Guo, X.~Qiu, P.~Liu, Y.~Shao, X.~Xue, and Z.~Zhang, ``Star-transformer,'' in
  \emph{NAACL-HLT}, 2019, pp. 1315--1325.

\bibitem{kitaev2020reformer}
N.~Kitaev, {\L}.~Kaiser, and A.~Levskaya, ``Reformer: The efficient
  transformer,'' \emph{arXiv:2001.04451}, 2020.

\bibitem{wang2020linformer}
S.~Wang, B.~Li, M.~Khabsa, H.~Fang, and H.~Ma, ``Linformer: Self-attention with
  linear complexity,'' \emph{arXiv:2006.04768}, 2020.

\bibitem{tay2020sparse}
Y.~Tay, D.~Bahri, L.~Yang, D.~Metzler, and D.-C. Juan, ``Sparse sinkhorn
  attention,'' \emph{arXiv:2002.11296}, 2020.

\bibitem{shen2018efficient}
Z.~Shen, M.~Zhang, H.~Zhao, S.~Yi, and H.~Li, ``Efficient attention: Attention
  with linear complexities,'' \emph{arXiv:1812.01243}, 2018.

\bibitem{katharopoulos2020transformers}
A.~Katharopoulos, A.~Vyas, N.~Pappas, and F.~Fleuret, ``Transformers are rnns:
  Fast autoregressive transformers with linear attention,''
  \emph{arXiv:2006.16236}, 2020.

\bibitem{kapur2017low}
S.~Kapur, A.~Mishra, and D.~Marr, ``Low precision rnns: Quantizing rnns without
  losing accuracy,'' \emph{arXiv:1710.07706}, 2017.

\bibitem{hou2018loss}
L.~Hou and J.~T. Kwok, ``Loss-aware weight quantization of deep networks,''
  \emph{arXiv:1802.08635}, 2018.

\bibitem{grachev2019compression}
A.~M. Grachev, D.~I. Ignatov, and A.~V. Savchenko, ``Compression of recurrent
  neural networks for efficient language modeling,'' \emph{Applied Soft
  Computing}, vol.~79, pp. 354--362, 2019.

\bibitem{damani20_pakdd}
S.~Damani, K.~N. Narahari, A.~Chatterjee, M.~Gupta, and P.~Agrawal, ``Optimized
  transformer models for faq answering,'' in \emph{PAKDD}, 2020, p. To appear.

\bibitem{yang2018accelerating}
Y.~Yang, K.~Liang, X.~Xiao, Z.~Xie, L.~Jin, J.~Sun, and W.~Zhou, ``Accelerating
  and compressing lstm based model for online handwritten chinese character
  recognition,'' in \emph{ICFHR}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2018, pp. 110--115.

\bibitem{lazaridou2013fish}
A.~Lazaridou, E.~M. Vecchi, and M.~Baroni, ``Fish transporters and miracle
  homes: How compositional distributional semantics can help np parsing,'' in
  \emph{EMNLP}, 2013, pp. 1908--1913.

\bibitem{wangperawong2018attending}
A.~Wangperawong, ``Attending to mathematical language with transformers,''
  \emph{arXiv:1812.02825}, 2018.

\bibitem{linzen2016assessing}
T.~Linzen, E.~Dupoux, and Y.~Goldberg, ``Assessing the ability of lstms to
  learn syntax-sensitive dependencies,'' \emph{TACL}, vol.~4, pp. 521--535,
  2016.

\bibitem{zaremba2014learning}
W.~Zaremba and I.~Sutskever, ``Learning to execute,'' \emph{arXiv:1410.4615},
  2014.

\end{thebibliography}

